FLStore: Efficient Federated Learning Storage for non-training workloads

Federated Learning (FL) is an approach for privacy-preserving Machine Learning (ML), enabling model training across multiple clients without centralized data collection. With an aggregator server coordinating training, aggregating model updates, and storing metadata across rounds. In addition to training, a substantial part of FL systems are the non-training workloads such as scheduling, personalization, clustering, debugging, and incentivization. Most existing systems rely on the aggregator to handle non-training workloads and use cloud services for data storage. This results in high latency and increased costs as non-training workloads rely on large volumes of metadata, including weight parameters from client updates, hyperparameters, and aggregated updates across rounds, making the situation even worse. We propose FLStore, a serverless framework for efficient FL non-training workloads and storage. FLStore unifies the data and compute planes on a serverless cache, enabling locality-aware execution via tailored caching policies to reduce latency and costs. Per our evaluations, compared to cloud object store based aggregator server FLStore reduces per request average latency by 71% and costs by 92.45%, with peak improvements of 99.7% and 98.8%, respectively. Compared to an in-memory cloud cache based aggregator server, FLStore reduces average latency by 64.6% and costs by 98.83%, with peak improvements of 98.8% and 99.6%, respectively. FLStore integrates seamlessly with existing FL frameworks with minimal modifications, while also being fault-tolerant and highly scalable.

==> Acknowledgments.tex <==
\section{Acknowledgments}

\new{We thank our shepherd, Sara Bouchenak, and our anonymous reviewers for their valuable feedback and suggestions. This work has been partially funded by NSF grants CSR-2106634, CSR-2312785, CCF-1919113, and OAC-2004751, along with UKRI-EPSRC grant EP/X035085/1.}

\vspace{10pt}

==> Discussion.tex <==
\section{Discussion and Limitations}
\label{sec:Discussion}

\paragraph{Support for Foundation Models.} Foundation Models are a class of models that have undergone training with a broad and general data set. Users can then fine-tune foundational models for specific use cases without training a model from scratch.
We have added and evaluated several foundation models from Figure~\ref{fig:model_footprint_per_request} in FLStore and continue to add more such models. We also add model inference as an application for FLStore with the aim of providing a cost-effective alternative for serving models efficiently compared to other cloud solutions such as AWS SageMaker~\cite{aws_sagemaker} which incurs high latency and costs as shown by our analysis in Figures~\ref{fig:total_time_breakup_comparison} and~\ref{fig:total_cost_breakup_comparison}.

% \subsection{Automating cache policy generation}
% \label{subsec:Automating cache policy generation}
% Our taxonomy of FL workloads and their associated caching policies is the result of a meticulously carried out study regarding the data requirements of these applications. However, our future work includes creating a system that can also work for other learning applications such as distributed large language model (LLM) training and other distributed deep learning (DL) applications. We envision a system that can create new caching policies at runtime for the non-training workloads of black-box distributed learning applications.
% \subsection{FLStore integration}
% \label{subsec:FLStore integration}
\paragraph{FLStore Integration.} Due to the modular nature of FLStore, it can be easily integrated into any existing FL framework. We have successfully integrated FLStore with IBMFL~\cite{ibmflgithub}, and FLOWER~\cite{beutel2020flower}, two popular FL frameworks used in industry and research.

% \subsection{Function memory limitations}
% \label{subsec:Function memory limitations}
\paragraph{Function Memory Limitations.} Serverless functions are limited in memory resources having a maximum of 10 GB memory~\cite{aws_lambda}. This is more than sufficient for handling non-training workloads for cross-device FL even for small transformer models such as~\cite{TinyLlama2024}. However, for even larger foundational models such as Large Language Models (LLMs)~\cite{NEURIPS2020_gpt3}, we are working on utilizing pipeline parallel processing where function groups can be assigned for each workload and each function in that group can perform computations in a pipeline parallel manner~\cite{serverlessML,INFless}.

Future work for FLStore includes adding further foundational models for all of these applications including XFL and model inference applications. We are also working towards the inclusion of automating workload detection for cache policy generation.
In particular, our current taxonomy of FL workloads and their associated caching policies is the result of a meticulously carried out study regarding the data requirements of these applications. However, future work includes creating a system that can also work for other learning applications such as distributed large language model (LLM) training and other distributed deep learning (DL) applications. We envision a system that can create new caching policies at runtime for the non-training workloads of black-box distributed learning applications.
